Degree Four Plane Spanners: Simpler and Better

Let ${\cal P}$ be a set of $n$ points embedded in the plane, and let ${\cal C}$ be the complete Euclidean graph whose point-set is ${\cal P}$. Each edge in ${\cal C}$ between two points $p, q$ is realized as the line segment $[pq]$, and is assigned a weight equal to the Euclidean distance $|pq|$. In this paper, we show how to construct in $O(n\lg{n})$ time a plane spanner of ${\cal C}$ of maximum degree at most 4 and stretch factor at most 20. This improves a long sequence of results on the construction of plane spanners of ${\cal C}$. Our result matches the smallest known upper bound of 4 by Bonichon et al. on the maximum degree of plane spanners of ${\cal C}$, while significantly improving their stretch factor upper bound from 156.82 to 20. The construction of our spanner is based on Delaunay triangulations defined with respect to the equilateral-triangle distance, and uses a different approach than that used by Bonichon et al. Our approach leads to a simple and intuitive construction of a well-structured spanner, and reveals useful structural properties of the Delaunay triangulations defined with respect to the equilateral-triangle distance. The structure of the constructed spanner implies that when ${\cal P}$ is in convex position, the maximum degree of this spanner is at most 3. Combining the above degree upper bound with the fact that 3 is a lower bound on the maximum degree of any plane spanner of ${\cal C}$ when the point-set ${\cal P}$ is in convex position, the results in this paper give a tight bound of 3 on the maximum degree of plane spanners of ${\cal C}$ for point-sets in convex position.

==> algo-fig.tex <==

\begin{figure}
\noindent
\begin{minipage}{.5\textwidth}
\centering

\begin{tikzpicture}[scale = 0.815]

\clip(-2.4,-2.7) rectangle (2.3,2.4);

\filldraw[fill=blue!10, draw=white] (0,0) -- ++(5cm,0mm) arc [start angle=0, end angle=60, radius=5cm] -- cycle;
\filldraw[fill=blue!10, draw=white] (0,0) -- ++(-5cm,0mm) arc [start angle=180, end angle=240, radius=5cm] -- cycle;

\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);

\draw (0,0) node[vertex,label=180:{$w$}] (w) {};
\draw (0.9105,-0.79449) node[vertex,label=0:{$v_0$}] (v0) {};
\draw (-0.52001,1.79464) node[vertex,label=90:{$v_1$}] (v1) {};
\draw (-1.67780,-1.49337) node[vertex,label=93:{$v_2$}] (v2) {};
\draw (-1.54,0.72) node[vertex,label=90:{$v_3$}] (v3) {};
\draw (1.66,1.18) node[vertex,label=90:{$v_4$}] (v4) {};
\draw (-0.56,-2.34) node[vertex,label=0:{$v_5$}] (v5) {};
%\draw (-1.6,-2.06) node[vertex,label=-93:{$v_6$}] (v6) {};

\draw [anchorEdge,dashed] (w) -- (v0);
\draw [anchorEdge,dashed] (w) -- (v1);
\draw [anchorEdge,blue] (w) -- (v2);
\draw [anchorEdge,dashed] (v3) -- (w);
\draw [anchorEdge,blue] (v4) -- (w);
\draw [anchorEdge,dashed] (v5) -- (w);
%\draw [anchorEdge] (v6) -- (v5);
\end{tikzpicture}

\centering (a)
\end{minipage}
\begin{minipage}{.5\textwidth}
\centering

\begin{tikzpicture}[scale = 1.3]

%[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-2.2,-5) rectangle (3,-1.8);

\filldraw[fill=blue!10, draw=white] (0,0) -- ++(5cm,0mm) arc [start angle=0, end angle=60, radius=5cm] -- cycle;
\filldraw[fill=blue!10, draw=white] (0,0) -- ++(-5cm,0mm) arc [start angle=180, end angle=240, radius=5cm] -- cycle;

\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);

\draw (0,0) node[vertex,label=90:{$w$}] (w) {};

\filldraw[fill=blue!10, draw=blue!30] (-1,-3.2) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (-1,-3.2) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-1,-3.2) node[vertex,label=180:{$p_7$}] (v) {};

\filldraw[fill=blue!10, draw=blue!30] (-0.62,-3.62) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (-0.62,-3.62) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-0.62,-3.62) node[vertex,label=225:{$p_6$}] (p6) {};

\filldraw[fill=blue!10, draw=blue!30] (-0.16,-4) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (-0.16,-4) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-0.16,-4) node[vertex,label=270:{$p_5$}] (p5) {};

\filldraw[fill=blue!10, draw=blue!30] (0.22,-3.52) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (0.22,-3.52) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (0.22,-3.52) node[vertex,label=90:{$p_4$}] (p4) {};

\filldraw[fill=blue!10, draw=blue!30] (0.76,-3.6) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (0.76,-3.6) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (0.76,-3.6) node[vertex,label=45:{$p_3$}] (p3) {};

\filldraw[fill=blue!10, draw=blue!30] (1.22,-4.08) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (1.22,-4.08) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (1.22,-4.08) node[vertex,label=225:{$p_2$}] (p2) {};

\filldraw[fill=blue!10, draw=blue!30] (1.76,-4.54) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (1.76,-4.54) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (1.76,-4.54) node[vertex,label=270:{$p_1$}] (p1) {};

\filldraw[fill=blue!10, draw=blue!30] (2.1,-4.02) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=blue!30] (2.1,-4.02) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (2.1,-4.02) node[vertex,label=-60:{$p_0$}] (p0) {};

\draw [shortcut] (p3)-- (p0);
\draw [shortcut] (v)-- (p4);

\draw [anchorEdge] (v) -- (w);
\draw [canonical] (v) -- (p6);
\draw [canonical] (p6) -- (p5);
\draw [canonical,color=blue] (p4) -- (p5);
\draw [canonical] (p4) -- (p3);
\draw [canonical] (p3) -- (p2);
\draw [canonical,-] (p2) -- (p1);
\draw [canonical,color=blue] (p0) -- (p1);

\end{tikzpicture}

\centering (b)
\end{minipage}

\caption{(a) $w$ is an example of a point that has, in $\dela$, an anchor in
every cone. Both blue anchors are added to the spanner in step 1; no more
than one white anchor in each white sector is added to the spanner. (b) An
illustration of step 6 of the algorithm.}
\label{fi:algorithm}

\end{figure}



==> algo-step.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}
%[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-2.2,-4.8) rectangle (3,1);

\filldraw[fill=blue!10, draw=white] (0,0) -- ++(5cm,0mm) arc [start angle=0, end angle=60, radius=5cm] -- cycle;
\filldraw[fill=blue!10, draw=white] (0,0) -- ++(-5cm,0mm) arc [start angle=180, end angle=240, radius=5cm] -- cycle;

\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);

\draw (0,0) node[vertex,label=90:{$w$}] (w) {};

\filldraw[fill=blue!10, draw=white] (-1,-3.2) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (-1,-3.2) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-1,-3.2) node[vertex,label=180:{$p_7$}] (v) {};

\filldraw[fill=blue!10, draw=white] (-0.62,-3.62) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (-0.62,-3.62) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-0.62,-3.62) node[vertex,label=225:{$p_6$}] (p6) {};

\filldraw[fill=blue!10, draw=white] (-0.16,-3.9) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (-0.16,-3.9) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (-0.16,-3.9) node[vertex,label=270:{$p_5$}] (p5) {};

\filldraw[fill=blue!10, draw=white] (0.22,-3.52) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (0.22,-3.52) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (0.22,-3.52) node[vertex,label=90:{$p_4$}] (p4) {};

\filldraw[fill=blue!10, draw=white] (0.76,-3.6) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (0.76,-3.6) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (0.76,-3.6) node[vertex,label=45:{$p_3$}] (p3) {};

\filldraw[fill=blue!10, draw=white] (1.22,-3.98) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (1.22,-3.98) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (1.22,-3.98) node[vertex,label=225:{$p_2$}] (p2) {};

\filldraw[fill=blue!10, draw=white] (1.76,-4.34) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (1.76,-4.34) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (1.76,-4.34) node[vertex,label=270:{$p_1$}] (p1) {};

\filldraw[fill=blue!10, draw=white] (2.1,-4.02) -- ++(3mm,0mm) arc [start angle=0, end angle=60, radius=3mm] -- cycle;
\filldraw[fill=blue!10, draw=white] (2.1,-4.02) -- ++(-3mm,0mm) arc [start angle=180, end angle=240, radius=3mm] -- cycle;
\draw (2.1,-4.02) node[vertex,label=-60:{$p_0$}] (p0) {};

\draw [shortcut] (p3)-- (p0);
\draw [shortcut] (v)-- (p4);

\draw [anchorEdge] (v) -- (w);
\draw [canonical] (v) -- (p6);
\draw [canonical] (p6) -- (p5);
\draw [canonical,color=blue] (p4) -- (p5);
\draw [canonical] (p4) -- (p3);
\draw [canonical] (p3) -- (p2);
\draw [canonical,-] (p2) -- (p1);
\draw [canonical,color=blue] (p0) -- (p1);

\end{tikzpicture}
\caption{Illustration of step 6 of the spanner construction.}
\label{fi:shortcuts}
\end{center}
\end{figure}



==> defns-fig.tex <==

\begin{figure}
\noindent
\begin{minipage}{.33\textwidth}
\centering
\begin{tikzpicture}[scale = 0.75]

\clip(-2.4,-2.7) rectangle (2.3,2.4);

%\filldraw[fill=blue!10, draw=white] (0,0) -- ++(5cm,0mm) arc [start angle=0, end angle=60, radius=5cm] -- cycle;
%\filldraw[fill=blue!10, draw=white] (0,0) -- ++(-5cm,0mm) arc [start angle=180, end angle=240, radius=5cm] -- cycle;

\filldraw[fill=black!5, draw=white] (0,0) -- ++(60:2.1) -- ++ (180:2.1) -- cycle;
\filldraw[fill=black!5, draw=white] (0,0) -- ++(0:1.4) -- ++ (-120:1.4) -- cycle;
\filldraw[fill=black!5, draw=white] (0,0) -- ++(-120:2.13) -- ++ (120:2.13) -- cycle;


\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);


\draw (0,0) ++(30:2.2) node {$-$};
\draw (0,0) ++(90:2.2) node {$+$};
\draw (0,0) ++(150:2.2) node {$-$};
\draw (0,0) ++(210:2.2) node {$+$};
\draw (0,0) ++(270:2.2) node {$-$};
\draw (0,0) ++(330:2.2) node {$+$};



\draw (0,0) node[vertex,label=30:{$w$}] (w) {};
\draw (0.9105,-0.79449) node[vertex,label=4:{$v_0$}] (v0) {};
\draw (-0.52001,1.79464) node[vertex,label=95:{$v_1$}] (v1) {};
\draw (-1.37780,-1.29337) node[vertex,label=-90:{$v_2$}] (v2) {};
%\draw (-1.54,0.72) node[vertex,label=90:{$v_3$}] (v3) {};
%\draw (1.66,1.18) node[vertex,label=90:{$v_4$}] (v4) {};
%\draw (-0.56,-2.34) node[vertex,label=0:{$v_5$}] (v5) {};
%\draw (-1.6,-2.06) node[vertex,label=-93:{$v_6$}] (v6) {};

\draw [canonical,black] (w) -- (v0);
\draw [canonical,black] (w) -- (v1);
\draw [canonical,black] (w) -- (v2);
%\draw [anchorEdge] (v3) -- (w);
%\draw [anchorEdge,blue] (v4) -- (w);
%\draw [anchorEdge] (v5) -- (w);
%\draw [anchorEdge] (v6) -- (v5);
\end{tikzpicture}

\centering (a)
\end{minipage}%
\begin{minipage}{.33\textwidth}
\centering

\begin{tikzpicture}[scale = 0.7]

%[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-2.2,-4.7) rectangle (3,0.9);

\filldraw[fill=black!5, draw=white] (0,0) -- ++(-120:3.7) -- ++ (0:3.7) -- cycle;


\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);

\draw (0,0) node[vertex,label=90:{$w$}] (w) {};

\draw (-2,-3.6) node[vertex,label=-90:{$v_1$}] (v1) {};
\draw (-1,-3.2) node[vertex,label=-90:{$v_2$}] (v) {};
\draw (-0.62,-3.62) node[vertex,label=-90:{$v_3$}] (v3) {};
\draw (-0.16,-4) node[vertex,label=-90:{}] (v4) {};
\draw (0.22,-3.52) node[vertex,label=90:{}] (v5) {};
\draw (0.76,-3.6) node[vertex,label=90:{}] (v6) {};
\draw (1.22,-4.08) node[vertex,label=-135:{}] (v7) {};
\draw (1.66,-4.44) node[vertex,label=-90:{}] (v8) {};
\draw (2.1,-4.02) node[vertex,label=0:{$v_k$}] (v9) {};

%\node [name path=vx,help lines,draw,] (v) -- ++(10,0){};
%\path [help lines,name path=vy] (v) -- ++(300:5);
%\path [help lines,name path=vx] (v) -- ++(0:5);



%\draw [help lines] (p0) -- ++(240:5);
%\draw [help lines] (p0) -- ++(60:5);
%\draw [help lines] (p6) -- ++(240:0.4);
%\draw [help lines] (p5) -- ++(240:0.7);
%\draw [help lines] (p4) -- ++(240:1.5);
%\draw [help lines] (p3) -- ++(240:2);
%\draw [help lines] (p2) -- ++(240:2);
%\draw [help lines] (p1) -- ++(240:2);
%\draw [help lines] (p1) -- ++(300:2);
%\draw [help lines] (p4) -- ++(300:3);
%\draw [help lines] (p5) -- ++(300:3);

%\path [help lines,name path=p0u] (p0) -- ++(60:2.4);
%\path [help lines,name path=p0l] (p0) -- ++(240:5);

%\path [name intersections={of=vx and p0u, by={Y}}];
%\path [name intersections={of=vy and p0l, by={Z}}];

%\draw [thick] (v) -- (Y) -- (Z) -- (v);

%\node	[name path=P7,draw, line through=(v)] ;

\draw [anchorEdge,black] (v) -- (w);
\draw [canonical,black] (v) -- (v1);
\draw [canonical,black] (v) -- (v3);
\draw [canonical,black] (v3) -- (v4);
\draw [canonical,black] (v5) -- (v4);
\draw [canonical,black] (v5) -- (v6);
\draw [canonical,black] (v6) -- (v7);
\draw [canonical,black] (v7) -- (v8);
\draw [canonical,black] (v9) -- (v8);


\draw [fan,black] (v1) -- (w);
\draw [fan,black] (v3) -- (w);
\draw [fan,black] (v4) -- (w);
\draw [fan,black] (v5) -- (w);
\draw [fan,black] (v6) -- (w);
\draw [fan,black] (v7) -- (w);
\draw [fan,black] (v8) -- (w);
\draw [fan,black] (v9) -- (w);
\end{tikzpicture}

\centering (b)
\end{minipage}%
\begin{minipage}{.33\textwidth}
\centering

\begin{tikzpicture}[scale = 0.9]

%[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-2.2,-6.6) rectangle (3,-2.4);


\draw (-5,0) -- (5,0);
\draw (0,0) -- (60:5); \draw (0,0) -- (240:5);
\draw (0,0) -- (120:5); \draw (0,0) -- (300:5);

\draw (0,0) node[vertex,label=90:{$w$}] (w) {};

\draw (-1,-3.2) node[vertex,label=180:{$x=v$}] (v) {};
\draw (-0.62,-3.62) node[vertex,label=180:{}] (p6) {};
\draw (-0.16,-4) node[vertex,label=90:{}] (p5) {};
\draw (0.22,-3.52) node[vertex,label=90:{}] (p4) {};
\draw (0.76,-3.6) node[vertex,label=45:{}] (p3) {};
\draw (1.22,-4.08) node[vertex,label=45:{}] (p2) {};
\draw (1.66,-4.44) node[vertex,label=0:{}] (p1) {};
\draw (2.1,-4.02) node[vertex,label=0:{$u$}] (p0) {};

%\node [name path=vx,help lines,draw,] (v) -- ++(10,0){};
\path [help lines,name path=vy] (v) -- ++(300:5);
\path [help lines,name path=vx] (v) -- ++(0:5);



%\draw [help lines] (p0) -- ++(240:5);
%\draw [help lines] (p0) -- ++(60:5);
\path [draw,help lines,name path=p6z] (p6) -- ++(240:0.4);
\path [draw,help lines,name path=p5z] (p5) -- ++(240:0.7);
\path [draw,help lines,name path=p4z] (p4) -- ++(240:1.5);
\path [draw,help lines,name path=p3z] (p3) -- ++(240:2);
\path [draw,help lines,name path=p2z] (p2) -- ++(240:2);
\path [draw,help lines,name path=p1z] (p1) -- ++(240:2.1);
\path [draw,help lines,name path=p1y] (p1) -- ++(300:0.5);
\path [draw,help lines,name path=p4y] (p4) -- ++(300:2.5);
\path [draw,help lines,name path=p5y] (p5) -- ++(300:2.5);

\path [help lines,name path=p0u] (p0) -- ++(60:2.4);
\path [help lines,name path=p0l] (p0) -- ++(240:5);

\path [name intersections={of=vx and p0u, by={[label=45:$y$]Y}}];
\path [name intersections={of=vy and p0l, by={[label=0:$z$]Z}}];

\path [draw,  name intersections={of=vy and p6z, by={P6Z}}];
\path [name intersections={of=vy and p5z, by={P5Z}}];
\path [name intersections={of=vy and p4z, by={P4Z}}];
\path [name intersections={of=vy and p3z, by={P3Z}}];
\path [name intersections={of=vy and p2z, by={P2Z}}];
\path [name intersections={of=vy and p1z, by={P1Z}}];

\draw [thick] (v) -- (Y) -- (Z) -- (v);

\draw [green, very thick] (v) -- (P5Z);
\draw [green, very thick] (P4Z) -- (P1Z);


\path [name intersections={of=p0l and p1y, by={P1Y}}];
\path [name intersections={of=p0l and p4y, by={P4Y}}];
\path [name intersections={of=p0l and p5y, by={P5Y}}];

\draw [blue, very thick] (p0)  -- (P1Y);
\draw [blue, very thick] (P4Y) -- (P5Y);

%\node	[name path=P7,draw, line through=(v)] ;

\draw [anchorEdge,black] (v) -- (w);
\draw [canonical,green] (v) -- (p6);
\draw [canonical,green] (p6) -- (p5);
\draw [canonical,color=blue] (p4) -- (p5);
\draw [canonical,green] (p4) -- (p3);
\draw [canonical,green] (p3) -- (p2);
\draw [canonical,green] (p2) -- (p1);
\draw [canonical,color=blue] (p0) -- (p1);
\end{tikzpicture}

\centering (c)
\end{minipage}

\caption{(a) To contruct graph $\dela$, every point $w$ chooses the shortest
edge, according to the $\dst$ distance, in every positive cone. (b) Edge
$(v_2,w)$ is the anchor of $w$ in the negative cone shown because it is the
shortest edge, according to the $\dst$ distance, among edges incoming to
$w$ in the cone; the path $v_1, \ldots, v_k$ is the canonical path of anchor
$(v_2,w)$. (c) Illustration of Lemma~\ref{lem:canonical-bound}.}
\label{fi:definitions}

\end{figure}


